Brain-on-Switch: Towards Advanced Intelligent Network Data Plane via NN-Driven Traffic Analysis at Line-Speed

The emerging programmable networks sparked significant research on Intelligent Network Data Plane (INDP), which achieves learning-based traffic analysis at line-speed. Prior art in INDP focus on deploying tree/forest models on the data plane. We observe a fundamental limitation in tree-based INDP approaches: although it is possible to represent even larger tree/forest tables on the data plane, the flow features that are computable on the data plane are fundamentally limited by hardware constraints. In this paper, we present BoS to push the boundaries of INDP by enabling Neural Network (NN) driven traffic analysis at line-speed. Many types of NNs (such as Recurrent Neural Network (RNN), and transformers) that are designed to work with sequential data have advantages over tree-based models, because they can take raw network data as input without complex feature computations on the fly. However, the challenge is significant: the recurrent computation scheme used in RNN inference is fundamentally different from the match-action paradigm used on the network data plane. BoS addresses this challenge by (i) designing a novel data plane friendly RNN architecture that can execute unlimited RNN time steps with limited data plane stages, effectively achieving line-speed RNN inference; and (ii) complementing the on-switch RNN model with an off-switch transformer-based traffic analysis module to further boost the overall performance. We implement a prototype of BoS using a P4 programmable switch as our data plane, and extensively evaluate it over multiple traffic analysis tasks. The results show that BoS outperforms state-of-the-art in both analysis accuracy and scalability.

==> DataPlaneDesign/ASIS.tex <==
\subsection{\label{subsec:downstream_processing} Downstream Processing}

\fixme{replace !!! with the name of model}

\fixme{!!!} deployed in the programmable switches can output the final classification result based on the statistics on the number of windows for each class. When the maximum number of windows is not greater than the threshold (i.e., the confidence is weak), a downstream server is needed to analyze the packet/flow in detail. The packets transmitting from the switch to the downstream server carry the following extra information: the final result, the confidence, the precise timestamp from the switch, and whether there is timeout or hash collision in $Flow Info$.

The \fixme{rightmost} part of Figure \ref{fig:deployment} describes the logic of the downstream server. When receiving a packet already classified with fair confidence, the server just apply the corresponding processing of the class to the packet. Otherwise, the packet should be classified by a complex model in this server. The complex model is executed by GPU, which means that the input data have to be batched in order to improve the overall performance. The information of the packet, including 5-tuple, packet length, and timestamp, is sent to the batches through a ring buffer. Meanwhile, the server processes the packet according to the cached classification result that is calculated from the former packets.

==> DataPlaneDesign/Algorithm.tex <==
\subsection{\label{subsec:algorithm} Integrated Data Plane Processing Logic}

\fixme{This section introduces the Integrated Data Plane Processing Logic with the algorithm like NetBeacon}


\begin{algorithm}[t]
    \caption{Data Plane Analysis Logic}
    \label{alg:data_plane}
    \DontPrintSemicolon
    \SetAlgoLined
    
    $idx \gets \mathcal{H}(5-tuple)[IndexWidth-1:0]$\;
    $ID \gets \mathcal{H}^{\prime}(5-tuple)[IDWidth-1:0]$\;
    $TS \gets timestamp[significant\ bits]$\;
    $ID_{stored},TS_{stored} \gets Reg_{PacketInfo}(idx)$\;
    \uIf{$TS-TS_{stored} \ge Threshold_{timeout}$}{
        $timeout \gets True$\;
        $collision \gets False$\;
        $Reg_{PacketInfo}(idx) \gets ID, TS$\;
    }\uElse{
        $timeout \gets False$\;
        \uIf{$ID=ID_{stored}$}{
            $collision\gets False$\;
            $Reg_{PacketInfo}(idx)\gets ID,TS$\;
        }\uElse{
            $collision\gets True$\;
        }
    }
    \BlankLine
    
    \uIf{$\neg collision$}{
        \uIf{$timeout$}{
            Init all $Regs(idx)$\;
            $IPD \gets 0$\;
        }\uElse{
            $IPD \gets TS-TS_{stored}$\;
        }
        
        $PacketCount \gets Reg_{PacketCount}(idx)$\;
        $Reg_{PacketCount}(idx) \gets PacketCount+1$\;
        
        $ev_S \gets FeatureEmbedding(IPD,packet\_length)$\;
        Get $ev_1$,...,$ev_{S-1}$ from $Regs_{ev}(idx)$\;
        Update $Regs_{ev}(idx)$ with $ev_S$ and $PacketCount$\;
        \uIf{$PacketCount<S$}{
            Per Packet Model\;
        }\uElse{
            $class_{window}\gets GRUs(ev_1,..,ev_S)$\;
            Update $Regs_{WindowCounter}(idx)$ with $class_{window}$\;
            \uIf{classification is obvious}{
                $class_{final}\gets class\ of\ most\ windows$\;
            }\uElse{
                Need further analysis\;
            }
        }
    }\uElse{
        Per Packet Model\;
    }
\end{algorithm}

\fixme{xht is overwhelmed here} 



==> DataPlaneDesign/Classifier_old.tex <==
% \subsection{\label{sec:classifier} Classifier}

% For each flow, the neural network continuously outputs the classification result based on the latest $L$ packets when each packet arrives. Fluctuations of classification results may occur when the user's behaviour changes or the model classifies wrongly. To ease the potential fluctuations, we deploy a classifier based on the statistics of past classification results. To be specific, assuming that there are $K$ results falling into $C$ classes and in the $i^{th}$ class there are $c_i$ results, where $1\le i\le C$, we pick out the class with most results, called $mx$. We set a threshold $f(K)$ and check whether $c_{mx}$ is greater than $f(K)$, if so, we take $mx$ as the final result, otherwise, a mark is set to notify downstream processing for detailed inspection.

% $K$ and $f(K)$ can be calculated parallelly with the model. After the model outputs the latest result, we allocate $C$ registers for each flow, corresponding to the counters of $C$ classes. The counters for $K$ and $c_i$ ($1\le i\le C$) are all $m$ bit(s) wide, reset every $2^m$ classification results.

% The core part of our classifier is selecting the maximum among $c_i$, where $1\le i\le C$, and compare it with the threshold $f(K)$. There are several ways to pick the maximum value. For instance, if there are two or more stages available, we can do subtraction between every two numbers at the first stage and then do ternary matching based on the sign bits with only $n$ entries. In our deployment, however, the number of stages are highly restricted. We advance an algorithm to select the maximum value within a single stage with ternary matching and calculate the number of entries required (see Appendix \ref{sec:appendix_select_maximum}). Also, we treat the threshold $f(K)$ as a candidate of the maximum value to save stages.


==> DataPlaneDesign/ControlPlane.tex <==
\subsection{\label{subsec:control_plane} Usage of Control Plane}

To ensure line-speed traffic analysis, \fixme{}

The model and flow management *DO NOT* need the cooperation with control plane during run time. The control plane is only responsible for installing the entries of tables (including $GRU$, $Output$, $Ebd$, $FC$, and $f$ in Figure \ref{fig:deployment}) at the very beginning. Also, when the model is retrained offline, the control plane can update the parameters through rewriting the table entries without a shutdown of the switch.

==> DataPlaneDesign/FlowManagement.tex <==
\subsection{Flow Management}
\label{subsec:flow_management} 

\sys relies on stateful storage to maintain per-flow state. 
Prior art~\cite{barradas2021flowlens, xing2020netwarden} relies on the control plane to allocate non-conflicting storage indices for different flows. 
To achieve line-speed traffic analysis, \sys relies on the readily available hardware hashing to allocate flow storage indices. 
In particular, the storage index for flow $f$ is computed as $\mathcal{H}(f(\textsf{5-tuple}) ~\%~ \textsf{N})$, where $\mathcal{H}$ is the hash function, and $\textsf{N}$ represents the total number of continuous per-flow storage blocks allocated for maintaining per-flow state. 

Both hash and modulo operations may result in flow index collisions, \ie two different flows (with different 5-tuples) may receive the same storage index. To avoid confusions, \sys stores a tuple $\{\textsf{TrueID}, \textsf{timestamp}\}$ alongside the storage index, where $\textsf{TrueID}$ represents the actual flow  identifier\footnote{To avoid resubmitting or recirculating packets, the read and write of the tuple need to be finished in an atomic operation. This restricts the length of $\textsf{TrueID}$ so that we cannot directly use 5 tuple as the $\textsf{TrueID}$. Thus, we leverage a different hash function $H^{\prime}$ to calculate the $\textsf{TrueID}$ as $H^{\prime}(f(\textsf{5-tuple}))$.} and \textsf{timestamp} represents the latest packet arrival time for the flow. 
When storage indices collide, \sys allows the new flow to take the occupied storage only if the existing flow is timed out (\ie the stored \textsf{timestamp} is earlier than a predefined threshold). Otherwise, the new arrived flow falls back to use the per-packet tree model trained using only per-packet features, or falls back to \imis; see discussions in \S~\ref{subsec:deepdive}. 

% This subsection describes how \fixme{!!!} manages the stateful storage for each flow in the data plane of the switch. The storage of a flow, like an element of an array, can only be accessed by an unique index owned by the flow, which is called the flow index. Prior arts (\eg FlowLens) rely on control plane to allocate indices for each flow, which is not suitable for line-speed traffic analysis. In the following part, we introduce our approach to the management of the flow index.

% \fixme{!!!} calculates the flow index based on hash function on the data plane. The expression of flow index can be described as $H(5-tuple)\%FLOW\_NUM$, where $H$ is a hash function. Hash function will inevitably encounter collisions, causing several flows to vie for the same position. To ease this problem, \fixme{!!!} manages the flows with a data structure called $Flow Info$. As shown in Figure \ref{fig:deployment}, in $Flow Info$, each flow stores its flow ID and latest timestamp (TS). When a packet arrives, the flow index and flow ID are calculated. \fixme{!!!} compares the timestamp of the arriving packet with the timestamp in $Flow Info$ to see whether the stored flow is out of date. If the stored flow is still alive, we check if two flow IDs are the same, or there is a hash collision.

% When a timeout happens (i.e., the stored flow is out of date), the old flow can no longer occupy the stateful resources. In this case, \fixme{!!!} replaces the stored ID and timestamp in $Flow Info$ with those of the new flow (i.e., the arriving packet). The stateful storage is also refreshed in the subsequent processing. When a hash collision happens (i.e., another active flow occupies the stateful resources), the new flow cannot use the stateful storage, and the analysis falls back on a per packet model. If there is neither timeout nor hash collision, \fixme{!!!} updates the timestamp in $Flow Info$.

% $Flow Info$ can be updated within itself without resubmitting or recirculating packets. In exchange, the full 5-tuple cannot be stored as flow ID due to the restrictions on stateful storage. Instead, \fixme{!!!} leverages another hash function $H^{\prime}$ to calculate $H^{\prime}(5-tuple)$ as the flow ID, minimizing the possibility of distraction between different flows (i.e., two different flows have a same ID).



% solution above faces difficulty in the flow management across the ingress and the egress. For instance, flow $a$ and flow $b$ do not encounter hash collision in their ingress pipelines $A$ and $B$ respectively, but they are forwarded to the same egress pipeline $C$ and have collision with each other. In this case, the stateful information stored in at least one side of $A$ and $B$ become meaningless, leading to the waste of the precious on-chip memory. Unless there is an one-to-one mapping between ingress pipelines and egress pipelines (i.e., the switch is treated as wires), the flow management will suffer from such cross-pipeline hash collision.

==> DataPlaneDesign/ModelDeployment.tex <==
\subsection{\label{subsec:model_deployment} Model Deployment}

\fixme{fix the name of the models}

%\fixme{Write the details on the data plane according to the section before. Also, some details are written in Implementations and a ref is needed}.

\fixme{Reorganize the description. remove the redundant part overlapping with above sections. The middle part of Figure Deployment is covered well in the above sections. The following points are new: \newline (i) The $last\_TS$ cannot be obtained from $FlowInfo$ and requires additional storage. But the $FlowInfo$ is mentioned in \ref{subsec:flow_management} and the detailed restrictions may be confidential. Currently, this point is mentioned in Section \ref{subsec:resource_usage}.\newline (ii) The details to embed the feature, like the width of $IPD$, $pkt\_len$ and the intermediate result before $FC$. Currently, the width of $TS$ (same as $IPD$) is listed in Section \ref{subsec:resource_usage}. The width of intermediate value, however, lacks discussion.\newline (iii) The details of storage of embedding vectors, as discussed in \ref{subsubsec:RNN_cell_and_output_layer} and \ref{subsec:impl_of_ev_storage}.\newline (iv) The optimization of the first and last $GRU$ and output layer, as discussed in Section \ref{subsubsec:RNN_cell_and_output_layer}. The problem why there are multiple $GRU$s is not discussed yet.\newline (v) Details of $WindowCounter$, as discussed in Section \ref{subsubsec:decision_making} and \ref{subsec:impl_of_decision_making}.\newline (vi) Details and optimization of $argmax$ and comparison with $threshold$, as discussed in Section \ref{subsec:impl_of_decision_making} and Appendix \ref{sec:appendix_select_maximum}.\newline (vii) Details of per packet model, which is not important and not discussed yet.}

As shown in the middle of Figure \ref{fig:deployment}, the deployment of \fixme{the model} can be divided into four main parts, namely feature embedding, RNN cell, output layer and decision making. The following sub-subsections will cover the deployment of each of these four parts.

\subsubsection{\label{subsubsec:feature_embedding}Feature Embedding}

This part is responsible for embedding the raw information, including the packet length and the inter-packet delay (IPD) into a condensed form of expression, as mentioned in the Line 4 in Algorithm \ref{alg:multi-level}. Firstly, \fixme{!!!} gets the timestamp of the last packet and calculates the IPD. Then, the packet length and IPD are embedded separately (denoted as $Ebd$ in Figure \ref{fig:deployment}). At last, a fully connected layer (denoted as $FC$) is applied to the results of embedding, getting $ev$, the embedding vector.

Note that the $Ebd$ and $FC$ are all implemented through match-action tables. For a $Ebd$ table, if the width of the input vector is not greater than that of the output vector, the table can be merged into $FC$ without extra costs.

\subsubsection{\label{subsubsec:RNN_cell_and_output_layer}RNN Cell and Output Layer}

According to Section \fixme{ref}, \fixme{!!!} feeds packets in a fixed-size sliding window to the binary RNN. Section \fixme{ref} explains that the embedding vectors of the last $S-1$ packets are stored, where $S$ is the size of the sliding window. As shown in Algorithm \ref{alg:multi-level}, a naive approach is that, for each flow, $S$ bins are allocated (indexed from $0$), and the $k^{th}$ packet stores its embedding vector in the $(k\%S)^{th}$ bin. \textbf{In fact, $S-1$ bins are enough for a flow.} The last time the embedding vector of $(k-S+1)^{th}$ packet is used is during the processing of the $k^{th}$ packet. After the $k^{th}$ packet obtains the embedding vector of $(k-S+1)^{th}$ packet, the storage can be reused. So, the $k^{th}$ packet applies the get-and-modify operation to the $(k\%(S-1))^{th}$ bin (indexed from $0$), storing its embedding vector and obtaining the embedding vector of the $(k-S+1)^{th}$ packet. The detailed implementation of the storage of embedding vectors is discussed in Section \ref{subsec:impl_of_ev_storage}.

To obtain the packet's sequence number, a packet counter is used (denoted as $Pkt Counter$ in Figure \ref{fig:deployment}). The packet count is also used to recognize the first $S-1$ packets of a flow, to which the \fixme{per packet model} is applied instead of the following neural network and decision making. The detailed implementation of the packet counter is introduced in Section \ref{subsec:impl_of_packet_count}.

The $GRU$s in Figure \ref{fig:deployment} are all implemented by 
match-action tables. The input vector of the $i^{th}$ $GRU$ is made up of the output vector of the $(i-1)^{th}$ $GRU$ ($0$ for the first) and the embedding vector of the $i^{th}$ packet in the sliding window (denoted as $ev_i$). Assuming that the length of output vector of $GRU$ is $a$ and the length of embedding vector is $b$, the first $GRU$ requires $2^{b}$ table entries and the rest require $2^{a+b}$ entries each. The action data of all the entries are $b$-bit width.

The output layer is a function that transform the output vector of the last $GRU$ to the classification result of the window. Assuming that there are $N$ classes, $\lceil log_2 N\rceil$ is far less than $a$, so the output layer and the last $GRU$ can be merged into a table with $2^{a+b}$ entries of $\lceil log_2 N\rceil$-bit width action data.

\subsubsection{\label{subsubsec:decision_making} Decision Making}

The \fixme{!!!} makes decisions according to the statistics of the number of windows of each classes. As described in Algorithm \ref{alg:multi-level}, the class of the most windows is picked and compared with a threshold to measure the confidence.

In deployment, for each class of each flow, a counter is allocated to count the number of windows of this class ($Window\ Counter\ 2$ in Figure \ref{fig:deployment}). The sum operation in Line 16 of Algorithm \ref{alg:multi-level} requires several stages. Instead, we allocate another counter for the total number of windows ($Window\ Counter\ 1$ in Figure \ref{fig:deployment}). The total number $K$ is independent from the neutral network above and can be obtained and updated once the packet count is confirmed to be greater than $S-1$. Also, the threshold $f(K)$ can be calculated beforehand. After the count of each class is obtained, the maximum value is picked through a ternary matching and then compared with the threshold. The details of implementation is discussed in Section \ref{subsec:impl_of_decision_making}.

%According to the sliding window described in \todo{Section XXX}, the output of the hidden layer is based only on the input of the current packet and the $L$ packets before it. It means that the hidden layer has only to remember the input from $L$ packets. If so, for a incoming packet, it can 

%In Figure \ref{fig:implementation}, $MemX$ represents the memory value based on the input of the latest $X$ packets and $Mem0$ is always $0$. $Func$ is the calculation function of one step of hidden layer. When processing the current packet, the new value of $MemX$ can be calculated from the old value of $Mem(X-1)$. The output of hidden layer, which is the value based on the input of the latest $L+1$ packets, can be calculated from the old value of $MemL$. So we can continuously produce the new output for each incoming packet.



%The model can be divided into four main parts, namely embedding layer, hidden layer, output layer and classifier, as shown in Figure \ref{fig:implementation}. The following sub-subsections will cover the implementation of each of these four parts.

%Before a packet is processed by the model, its flow index (denoted as $idx$ in Figure \ref{fig:implementation}), timestamp (denoted as $TS$), and packet length are already available. The output of the whole model is consists of the final classification result and/or whether further inspection is needed.

%\subsubsection{Embedding Layer}

%The target of the embedding layer is to embed the raw information of packets, packet length and time interval, into the input of the hidden layer (named $info$ in Figure \ref{fig:implementation}). Firstly, we get the timestamp of the last packet and calculate the time interval. Then, the packet length and time interval are embedded separately (denoted as $Ebd$ in Figure \ref{fig:implementation}). At last, a fully connected layer is applied to the results of embedding, getting $info$, the input of hidden layer.

%\subsubsection{Hidden Layer}

%According to the sliding window described in \todo{Section XXX}, the output of the hidden layer is based only on the input of the current packet and the $L$ packets before it. It means that the hidden layer has only to remember the input from $L$ packets. If so, for a incoming packet, it can 

%In Figure \ref{fig:implementation}, $MemX$ represents the memory value based on the input of the latest $X$ packets and $Mem0$ is always $0$. $Func$ is the calculation function of one step of hidden layer. When processing the current packet, the new value of $MemX$ can be calculated from the old value of $Mem(X-1)$. The output of hidden layer, which is the value based on the input of the latest $L+1$ packets, can be calculated from the old value of $MemL$. So we can continuously produce the new output for each incoming packet.

%\subsubsection{Output Layer}

%The output layer has only a fully connected layer that transforms the output of the hidden layer to the classification result.

%\subsubsection{Classifier}

%Every sliding window (\todo{see sec XXX}) will get a classification result from the output layer. The classifier counts the number of results $K$ and counting the (same as the number of sliding windows), 
%For each flow, the neural network continuously outputs the classification result based on the latest $L$ packets when each packet arrives. Fluctuations of classification results may occur when the user's behaviour changes or the model classifies wrongly. To ease the potential fluctuations, we deploy a classifier based on the statistics of past classification results. To be specific, assuming that there are $K$ results falling into $C$ classes and in the $i^{th}$ class there are $c_i$ results, where $1\le i\le C$, we pick out the class with most results, called $mx$. We set a threshold $f(K)$ and check whether $c_{mx}$ is greater than $f(K)$, if so, we take $mx$ as the final result, otherwise, a mark is set to notify downstream processing for detailed inspection.

%$K$ and $f(K)$ can be calculated parallelly with the model. After the model outputs the latest result, we allocate $C$ registers for each flow, corresponding to the counters of $C$ classes. The counters for $K$ and $c_i$ ($1\le i\le C$) are all $m$ bit(s) wide, reset every $2^m$ classification results.

%The core part of our classifier is selecting the maximum among $c_i$, where $1\le i\le C$, and compare it with the threshold $f(K)$. There are several ways to pick the maximum value. For instance, if there are two or more stages available, we can do subtraction between every two numbers at the first stage and then do ternary matching based on the sign bits with only $n$ entries. In our deployment, however, the number of stages are highly restricted. We advance an algorithm to select the maximum value within a single stage with ternary matching and calculate the number of entries required (see Appendix \ref{sec:appendix_select_maximum}). Also, we treat the threshold $f(K)$ as a candidate of the maximum value to save stages.


==> DataPlaneDesign/Model_old.tex <==
% \subsection{\label{sec:model} Model}

% Traditional RNN cannot be deployed due to the strict restrictions on the usage of stateful memory of switches. RNN requires ‘memory’, which is implemented with registers. One step of the hidden layer of RNN consists of a series of operations: (i) reading prior information from ‘memory’, (ii) calculating new information with prior information and input value, (iii) writing new information back to ‘memory’. The operation (i) and (iii) access the same register, forcing the whole process into a single stage, which is far beyond the capability of switches.

% A natural idea is to unfold the hidden layer of RNN and truncate the length of memory. To to specific, we denote the memory calculated from the $i^{th}$ to the $j^{th}$ packet as $mem_{i,j}$, where $1\le i\le j\le i+L$ and $L$ is the length of packet sequence the model can memory. Note that $mem_{i,i+L}$ is not really memorized. Also, we denote the information of the $i^{th}$ packet as $info_i$ ($i\ge 1$), which is calculated through embedding. One step of hidden layer can be written as $mem_{i,j+1}=Func(mem_{i,j}, info_j)$, where $1\le i\le j\le i+L-1$ and $Func$ represents the calculation function. 

% The storage of $mem_{i,j}$ is implemented by registers, denoted as $Mem_{j-i+1}$, where $1\le i\le j\le i+L-1$. When accessing $Mem_{k}$ during processing the $i^{th}$ packet, we get $mem_{i-k,i-1}$ and replace it with $mem_{i-k+1,i}$ through a get-and-modify operation ($i\ge 1, 1\le k\le L-1$), preventing the duplicate access to a same register.

% We realize the embedding layer and $Func$ by lookup tables, taking the input vector as key and the output vector as value. These lookup tables can be realized by either match-action tables or registers. For both approaches, the space overhead has an exponential relationship with the size of the input vector, so the bit width of $mem$ and $info$ cannot be large.

% For the $i^{th}$ packet of a flow, $info_i$ is calculated by embedding at first, followed by the calculation of $mem_{i,i}$, $Mem_1$, $Func$, $Mem_2$, $Func$, and so on, stage by stage. Finally we get the $mem_{i-L,i}$ and feed it to a fully connected layer for the classification result.

% In fact, the calculation of $mem_{i,i}$ from $info_i$ is redundant because we can directly get $mem_{i,i}$ through embedding, just like $info_i$. Also, the calculation of $mem_{i-L,i}$ and the output layer can be merged into a single lookup table, because $mem_{i-L,i}$ is no longer needed in the processing of later packets. 

% In conclusion, the model will take $2L$ stages to output the result after we have done the embedding, namely $Mem_1$, $Func$, $Mem_2$, $Func$,... , $Mem_L$, and $output$.



==> DataPlaneDesign/deprecated.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/fig argmax_table.png}
    \caption{\label{fig:argmax} \fixme{To be named}.}
\end{figure}

The number of entries follows the recurrence relation.

\begin{equation}
D(n,m)=2*D(n,m-1)+\sum_{i=1}^{n-1}\binom{n}{i}D(i,m-1),n\ge 2,m\ge 2
\end{equation}

\begin{equation}
D(n,1)=n,n\ge 1
\end{equation}

\begin{equation}
D(1,m)=1,m\ge 1
\end{equation}

The general term formula is not easy to solve, but we can see its performance through specific values. \fixme{Fix it after xht solves successfully.} For example, $D(5,5)=10245$ and $D(4,8)=44028$, which are far smaller than the $2^{5*5}$ and $2^{4*8}$ of the naive enumeration.

The above idea makes a great progress from the naive idea, but it is not enough, because table of $n=m=5$ still cannot be fit into one stage.

Our approach compresses the table with wildcards. When enumerating the highest bits, instead of listing all the $2^n$ situations, we firstly enumerate the cases with both `0'(s) and `1'(s), then we can merge the case of all `0's and all `1's together with a wildcard, as shown in the right part of Figure \ref{fig:argmax}.

It looks like we only do one merge, but the effect is huge. The new recurrence relation is shown as follow.

\begin{equation}
F(n,m)=F(n,m-1)+\sum_{i=1}^{n-1}\binom{n}{i}F(i,m-1),n\ge 2,m\ge 2
\end{equation}

\begin{equation}
F(n,1)=n,n\ge 1
\end{equation}

\begin{equation}
F(1,m)=1,m\ge 1
\end{equation}

We calculate the general term formula and it turns out to be $nm^{n-1}$ (details in Appendix \ref{sec:appendix_select_maximum}). In comparison with the method before merging entries, $F(5,5)=3125<10245$, and $F(4,8)=2048<44028$, in both cases one stage is enough for the table.

For the larger $n$ and/or $m$, we can divide the numbers into several groups, applying argmax in each group in the first stage and then applying argmax to all the winners of every groups in the second stage, fully utilizing the capability of parallel computations of the switch hardware, so the capabilities of our approach can be greatly expanded by an extra stage.

\fixme{In implementation, the parallel comparison in groups mentioned above is not used due to $n$ is not large. Also, there may be some restrictions other than TCAM, like crossbar, Packet Header Vector (PHV), and so on. So xht thinks the detailed description should be avoided.}

\fixme{xht stops here}
% The second key point is the argmax operation in decision making. Argmax is used to select the index of the maximum value in a given list. A python programmer can easily call the function np.argmax(), while a C programmer has to implement it with a loop. Argmax is not a primitive in p4 or switch hardware and needs to be designed. If there are multiple numbers tied for the maximum, argmax returns the first one.


% The naive idea to simulate the loop in C language, i.e., compare the first with the second, then compare the winner with the third, and so on. Denoting the number of candidates of argmax as $n$, this idea does $n-1$ comparisons sequentially and takes $n-1$ stages, which is not affordable.

Although picking the maximum among $n$ numbers cannot be done with less than $n-1$ comparisons, these comparisons do not have to be done in sequence. Like a single-elimination tournament, in each round (i.e., stage), each candidate competes (is compared) with another, and the winners (the greater ones) goes to the next round (stage). This approach leverages the capability of parallel computations in switch hardware. The total number of stages is decreased to $\lceil log_2 n\rceil$.

Before taking a step further, we must first understand how to implement the `compare' operation between two numbers (denoted as num$_A$ and num$_B$) in the switch hardware.
The statement
\begin{verbatim}
if (num_A > num_B) act_A; else act_B;
\end{verbatim}
cannot be successfully compiled because the condition is too complex.
There are two alternative approaches.
The first is dividing the above statement into 
\begin{verbatim}
tmp = num_A - num_B;
if (tmp > 0) act_A; else act_B;
\end{verbatim}
The second is designing a match-action table which takes the num$_A$ and num$_B$ as keys and does the act$_A$ or act$_B$ according to the key lookup.

When designing the table, a naive enumeration of num$_A$ and num$_B$ wastes too much space. In fact, if the highest bits of num$_A$ and num$_B$ are different, then we don't care about the rest bits, otherwise, we check the second highest bits, and so on. Note that the subsequent processes are the same when the highest bits are both '0' and both '1', so we can leverage wildcards to cover both these two cases. A corner case is there is only one bit remaining for both num$_A$ and num$_B$. Assuming that A has the higher priority than B (i.e., choose A when num$_A$=num$_B$), we can judge whether num$_A$ is '0' and num$_B$ is '1' (i.e., the winning case of B), if so (i.e., num$_B$ is greater), we choose B, otherwise (i.e., num$_A$ is greater, or there is a tie), we choose A. A table to compare two 2-bit width numbers is shown as follow (wildcard is denoted as 'x').

\begin{center}
    \begin{tabular}{||c c c||}
        \hline
        num$_A$ & num$_B$ & winner \\ [0.5ex] 
        \hline\hline
        1x & 0x & A \\ 
        \hline
        0x & 1x & B \\ 
        \hline
        x0 & *1 & B \\ 
        \hline
        xx & xx & A \\
        \hline
    \end{tabular}
\end{center}

The design of table can be generalized to implementing the argmax operation. The problem can be defined as follow: designing a ternary-match table that picks the maximum among $n$ keys of $m$-bits width each, selecting the first one if there is a tie for maximum value. The above case can be seems as $n=2$.

At first, we check the highest bit of each number. If there are some `1'(s) and some `0'(s), then we pick the maximum among the number(s) with '1' with $m'=m-1$. Otherwise, the bits are all '0' or all '1', we merge these two cases with wildcard and continue with $m'=m-1$. Anyway, the size of the problem ($m$ and/or $n$) becomes smaller, so we can solve it through recursive function. There are two corner cases: (i) $n=1$. There is only one number remaining, so an entry full of wildcards is enough. (ii) $m=1$. We design a table as follow.



The number of entries generated through the algorithm above, denoted as $F(n,m)$, is $nm^{n-1}$. We obtain this result from the recurrence relations corresponding to the recursive process of the algorithm. $F(n,m)=F(n,m-1)+\sum_{i=1}^{n-1}\binom{n}{i}F(i,m-1),n\ge 2,m\ge 2$, where $i$ enumerate the number of '1's in the highest bits. The initial conditions are $F(n,1)=n,n\ge 1$ and $F(1,m)=1,m\ge 1$. The proof and derivation are given in Appendix \ref{sec:appendix_select_maximum}.

With the algorithm above, we can implement argmax within one stage as long as the $n$ and $m$ are not large (e.g. $n=5,m=5$). For the larger $n$ and/or $m$, we can divide the numbers into several groups, applying argmax in each group in the first stage and then applying argmax to all the winners of every groups in the second stage, so the capabilities of our algorithm can be greatly expanded by an extra stage.

\fixme{Something about threshold may be added after the design is confirmed.}


%In the light of this, we compare between every two numbers in the first stage, and then get the maximum according to the $\frac{n(n-1)}{2}$ relationships with TCAM... // after coding on Tofino, only n<=5 is OK, limited by PHV resouces when n>=6

\SetKwComment{Comment}{$\triangleright$~}{}
\SetKwInOut{KwIn}{Define}
\begin{algorithm}[t]
    \caption{Argmax table entry generation}
    \label{alg:argmax}
    \DontPrintSemicolon
    % \SetAlgoLined

    \KwIn {$n$: \# of keys; $m$: the bit width of each key}

    $S, \textsf{entry}\gets \{1,...,n\}, [... , ..., ...]$ \Comment*{\g{n m-bit segments }}
    % $\textsf{Work}(S, m, \textsf{entry})$ \;
    \hline
    \textbf{Procedure}: Iterate$(S, m, entry)$\;
    \lIf {$m=1$}{\textsf{Generate} (S, \textsf{entry}) and exit} 
    \For {$\Phi\subsetneqq S^{\prime}\subsetneqq S:$} {
        $\textsf{entry}^{\prime}=\textsf{entry}$ \;
        for $i\in S\setminus S^{\prime} \xrightarrow{} \textsf{entry}^{\prime}[i]+=`0'+`**...*'$ \Comment*{\g{$(m-1) \times `*'$}}
        for $i\in S^{\prime} \xrightarrow{} \textsf{entry}^{\prime}[i]+=`1'$\;
        $\textsf{Work}(S^{\prime}, m-1, \textsf{entry}^{\prime})$\Comment*{\g{some 0 and some 1}}
    }
    $\textsf{entry}^{\prime}[i]=\textsf{entry}[i]$ \;
    for $i\in S \xrightarrow{} \textsf{entry}^{\prime}[i]+=`0'$\;
    $\textsf{Work}(S, m-1, \textsf{entry}^{\prime})$\Comment*{\g{all 0 or all 1}}
    return \;
    \hline
    Procedure: Output$(S, entry)$\Comment*{\g{case $m=1$}}
    $a=\textsf{list}(S)$ from LOW priority to HIGH priority\;
    \For {$i=0$ to $\textsf{len}(a)-1$} {
        $\textsf{entry}^{\prime}=\textsf{entry}$ \;
        for $k<i \xrightarrow{} \textsf{entry}^{\prime}[a[k]]+=`*'$ \;
        for $k>i \xrightarrow{} \textsf{entry}^{\prime}[a[k]]+=`0'$ \;
        $\textsf{entry}^{\prime}[a[i]]+=`0'$ \;
        $\textsf{print}(\textsf{entry}^{\prime},\textsf{winner}=a[i])$\Comment*{\g{print entry}}
    }
    return\;
\end{algorithm}



==> Implementation/ActualCase.tex <==
\subsection{\label{subsec:actual_case}Actual Case}

\subsubsection{\label{subsubsec:hyper-parameters}Hyper-parameters}

In our implemented prototype, the hyper-parameters are listed below.

\begin{center}
    \begin{tabular}{||c c||}
        \hline
        hyper-parameter & value \\ [0.5ex] 
        \hline\hline
        Window Size (S) & 8 \\ 
        \hline
        Number of Classes (N) & 5 \\
        \hline\hline
        Bit Width of Embedded Length & 10 \\
        \hline
        Bit Width of Embedded IPD & 8 \\
        \hline
        Bit Width of Embedding Vector & 6 \\
        \hline
        Bit Width of Hidden State & 12 \\
        \hline\hline
        Reset period of Window Counter & 32 \\
        \hline
        Bit Width of Intermediate Probability & 4 \\
        \hline
        Bit Width of Cumulative Probability & 9 \\
        \hline\hline
        Bit Width of $ID$ & 32 \\
        \hline
        Bit Width of $TS$ & 32 \\
        \hline
        $MAX\_FLOW\_NUM$ & 65536 \\
        \hline
    \end{tabular}
\end{center}

The bit width of cumulative probability is calculated from the product of reset period of window counter and the maximum value of intermediate probability, which effects the argmax operation.

\subsubsection{\label{subsubsec:stage usage}Stage Usage}

\fixme{Important: The actual case of stage usage is different from the ideal case. Firstly, the model cannot be implemented within ingress pipeline due to the limitation of stages, which means both ingress and egress are used ($12+12$ stages). Secondly, the ingress and egress share the hardware resources. For instance, if a stage in ingress costs most of SRAM, then the corresponding stage in egress can use only a little SRAM, leading to the split of tables. Also, the number of registers (register arrays) in each stage is limited. Only 4 registers (register arrays) are allowed in one stage, and the amount is shared by the ingress and egress. Finally, for the argmax operation, the table generated for $n=5,m=9$ takes much more TCAM than a stage has, so we split the argmax to two $n=3,m=9$ in sequence, i.e., firstly compare the first three numbers, then compare the winner and the other two numbers. }

The actual stage usage is listed below. We use all the stages in both ingress and egress pipeline. The detailed resource consumption of each component is discussed in Section \fixme{ref evaluation}.

\begin{center}
    \begin{tabular}{|| c | c | c ||}
        \hline
        stage & ingress & egress \\ [0.5ex] 
        \hline\hline
        0 & \makecell{$\textsf{calculate}\ ID,\ idx$,\\ \textsf{embed\ pkt\ length}} & \makecell{$GRU_4$, \\$WindowCounter$} \\ 
        \hline
        1 & $FlowInfo$ & $GRU_5$ \\ 
        \hline
        2 & \makecell{$pkt\_counter1$, \\$pkt\_counter2$, \\$last\_TS$} & \makecell{$GRU_5$, \\$\textsf{calculate\ threshold}$} \\ 
        \hline
        3 & $\textsf{calculate\ IPD}$ & $GRU_6$ \\ 
        \hline
        4 & $\textsf{embed\ IPD}$ & $GRU_7$ \\ 
        \hline
        5 & $FC$ & $GRU_8$ \\ 
        \hline
        6 & $bin_{4,5,6,7}$ & $GRU_8$ \\ 
        \hline
        7 & $bin_{1,2,3}$ & $cnt_1$ \\ 
        \hline
        8 & $\textsf{dispatch\ ev}$ & \makecell{$cnt_{2,3,4,5}$} \\ 
        \hline
        9 & $GRU_1$ & $t\gets\textsf{argmax}(cnt_{1,2,3})$ \\ 
        \hline
        10 & $GRU_2$ & $\textsf{argmax}(t,cnt_{4,5})$\\ 
        \hline
        11 & $GRU_3$ & $\textsf{EscalationMark}$ \\ 
        \hline
    \end{tabular}
\end{center}




==> Implementation/IdealCase.tex <==
\subsection{\label{subsec:ideal_case}Ideal Case}

\iffalse
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{images/fig dependency.png}
    \caption{\label{fig:dependency} The simplified dependency and the minimum number of stages required.}
\end{figure*}
\fi

Figure \ref{fig:dependency} shows the simplified dependency graph of the components of \fixme{name}. In this graph, if there are dependencies $a\xrightarrow{} b$ and $\xrightarrow{}c$, then $a\xrightarrow{} c$ is not displayed. The red arrow represents control dependency, while the black arrow represents data dependency. In the ideal case (i.e., the hyper-parameters of the model are small), the numbers of stages required of each component are written in the brackets.

\fixme{Important: When a packet arrives, we first apply the flow management to this packet, including the calculation of flow ID and flow index in the first stage and the judgment of hash collision or timeout with FlowInfo in the second stage (as described in Section \ref{subsec:flow_management}). If there is no hash collision, then it takes three stages to get the embedded value of inter-packet delay (IPD), namely the storage of the last timestamp, the subtraction for IPD, and the embedding of IPD.} The embedding of packet length is not restricted by the flow management can be done anywhere before the fully connected layer which compresses the embedded value of length and IPD into a embedding vector. Then we store the embedding vector of the current packet, get the embedding vectors of the packets in the current segment and dispatch them to proper GRU tables (see Section \ref{subsubsec:embedding_vector_storage}), with the help of the counters described in Section \ref{subsubsec:counters}.
If the packet is not the first $S$ packets of a flow, we execute $S$ RNN time steps, i.e., $S$ GRU tables sequentially and get the intermediate result (the class and the probability) through the output layer. We accumulate the probability for each class, and get the class with the highest cumulative probability as the final classification through argmax operation discussed in Section \ref{subsubsec:decision_making}. Finally, the maximum cumulative probability is compared with a class-specific threshold multiplied by the window counter, measuring whether the confidence is low or not. If the the confidence is low, then this packet and all the following packets of this flow should be sent to escalated analysis. The mark of escalating or not is stored in the last component of the whole work flow. 

\fixme{Important: The per packet model has little side effect on the implementation of out model, because (i) the per packet model mainly uses TCAM resource, while the main part of our model uses SRAMs only, except the argmax (see Section \ref{subsubsec:decision_making}), and (ii) no component of our model depends on the per packet model. So we do not care much about the per packet model.}

\fixme{Important: The critical path starts at Flow Management at the top and goes straight down to the argmax and the comparison for confidence, and finally to the storage of the escalation mark, taking $(13+S)$ stages in ideal.}

\fixme{Important: \parab{Optimization} There are two optimizations on the basis of Figure \ref{fig:dependency}: (i) The table of output layer is merged with the last GRU table (GRU$_S$), i.e., $C=\textsf{Output}(\textsf{GRU}_S(h,ev_S)) \xrightarrow{merge} C=(\textsf{Output}\circ\textsf{GRU}_S)(h,ev_S)$. (ii) The comparison between the maximum cumulative probability and the corresponding threshold can be divided into a subtraction and a comparison with $0$ (or a check for the sign bit). The subtraction can be done in the action of the winning case of each class in the match-action table of argmax. And the comparison with $0$ can be done within the atomic operation of updating and getting the escalation mark. The above two optimizations save a total of two stages, which is conducive to the actual implementation.}



==> Implementation/ImplementationOfDecisionMaking.tex <==
\subsection{\label{subsec:impl_of_decision_making} Implementation of Decision Making}

%This section introduces the reset period of window counters and the more detailed way to select maximum, ?the optimization through treat threshold as one candidate of maximum
%no pseudo code of P4 due to this section is already too large

As introduced in Section \ref{subsubsec:decision_making}, each flow is equipped with $N+1$ window counters ($N$ is the number of classes), one for the total number of windows and the rest count windows of each class. All the window counters are $m$ bit(s) wide, reset every $2^m$ windows. 

The core part of decision making is selecting the maximum value among the counts of $N$ classes. A naive idea is leverage the if-else nesting. Sadly, the hardware only supports comparison with constants in conditional branches. An alternative approach is to do subtraction between every pair of counts at first and then pick the maximum based on the sign bits through if-else nesting or a ternary matching with $N$ entries, which takes 2 stages. To save stages, we advance an algorithm to select the maximum value within a single stage with ternary matching and calculate the number of entries required.

We define the problem as following conditions and restrictions.

\begin{enumerate}
\item There are $n$ numbers of $m$ bit(s) each, where $n,m\ge 1$.
\item There is a predefined order to determine which number to select when there is a tie for maximum value.
\item Only one ternary matching is allowed, i.e., the calculation before matching is prohibited.
\end{enumerate}

We advance an algorithm to design the entries of ternary matching. Firstly, there are two naive cases. For $n=1$, only one entry (i.e., all wildcards) is needed. For $m=1$, we need $n$ entries, i.e., enumerate the winning case of each number in predefined reverse order. For other cases, we first compare the most significant bits and (i) weed out some of the numbers, or (ii) ignore this bit when all bits are equal. Then the problem is reduced to a sub-problem with $m'=m-1$.

We denote the number of required entries based on our algorithm as $F(n,m)$. The conclusion is that $F(n,m)=nm^{n-1}$. The proof and derivation process is provided in Appendix \ref{sec:appendix_select_maximum}.

Also, we treat the threshold $f(K)$ as a candidate of the maximum value to save one stage at the cost that if the threshold is the maximum (i.e., the confidence is weak), the final classification result cannot be obtained.


==> Implementation/ImplementationOfEVStorage.tex <==
\subsection{\label{subsec:impl_of_ev_storage} Implementation of Embedding Vector Storage}

%This section introduces the implementation of the storage of ev,  with the pseudo code of P4
\fixme{Unify the name of 'packet sequence number' or 'packet index' or 'packet count'}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/fig p4_ev_storage.png}
    \caption{\label{fig:p4_ev_storage}  P4 pseudo-code for storage of embedding vector.}
\end{figure}

As discussed in Section \ref{subsubsec:RNN_cell_and_output_layer}, \fixme{!!!} allocates $S-1$ bins (indexed from $0$) for each flow to store the embedding vectors ($S$ is the size of the sliding window). The $k^{th}$ packet of a flow stores its embedding vector in the $(k\%(S-1))^th$ bin. In a sliding window, we denote the embedding vector of the $i^{th}$ packet as $ev_i$, where $i$ is the sequence number \textbf{in this window} ($1\le i\le S$) and $ev_1$ to $ev_S$ forms the input sequence of $GRU$s.

During the processing of the $k^{th}$ packet, the sliding window to process covers from the $(k-S+1)^{th}$ packet to the $k^{th}$ packet. The problem is that, $ev_i$ ($1\le i\le S-1$) is previously stored in the $((k-S+i)\%(S-1))^{th}$ bin, so the matches between bins and $ev_i$s change with the packet count $k$. The values read from bins are firstly stored into temporary space in metadata, and then the order is adjusted according to $k\%(S-1)$, because $k$ and $k^{\prime}=k+S-1$ have the same effect. The above process is shown in Figure \ref{fig:p4_ev_storage}.

==> Implementation/ImplementationOfPacketCount.tex <==
\subsection{\label{subsec:impl_of_packet_count} Implementation of Packet Count}

%This section introduces the implementation of the packet count, with the pseudo code of P4

\fixme{Unify the name of 'packet sequence number' or 'packet index' or 'packet count'}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/fig p4_packet_counter.png}
    \caption{\label{fig:p4_packet_counter}  P4 pseudo-code for packet counter.}
\end{figure}

The packet count is used in two places. The first is to recognize the first $S-1$ packets of a flow (S is the size of the sliding window). These packets get their classification results through the \fixme{per packet model}, because the first window is not filled up yet. The second is to assist the storage of the embedding vectors $ev$, where the $packet_count\%(S-1)$ is calculated, as described in Section \ref{subsubsec:RNN_cell_and_output_layer}.

A naive approach that implements a packet counter at first and then compares with $S$ and does modulo operation is not feasible, because the bit width of the counter should be limited.

\fixme{!!!} implements two counters to solve this problem, as shown in Figure \ref{fig:p4_packet_counter}. The first counter is increased from $1$, and stopped at $S$. For the $i^{th}$ packet, the counter returns $i$ when $i<S$, otherwise returns $S$. The second counter is increased from $0$ and returns back to $0$ after $S-2$, simulating the modulo operation. The first counter helps to recognize the first $S-1$ packets, while the second counter provides the remainder.

==> Implementation/ResourceUsage.tex <==
\subsection{\label{subsec:resource_usage} Resource Usage}

This subsection reports the hyper-parameters of the prototype. It also reports the resource cost of each main component separately. Finally, the stage usage is displayed.
\iffalse
\subsubsection{hyper-parameters}
In our implemented prototype, the hyper-parameters are listed below.

\begin{center}
    \begin{tabular}{||c c||}
        \hline
        hyper-parameter & value \\ [0.5ex] 
        \hline\hline
        Window Size (S) & 8 \\ 
        \hline
        Class Number (N) & 5 \\
        \hline
        Width of Embedding Vector ($|ev|$) & 6 \\
        \hline
        Width of Hidden State ($|h|$) & 12 \\
        \hline
        Width of Window Counter & 5 \\
        \hline
        Width of $ID$ & 32 \\
        \hline
        Width of $TS$ & 32 \\
        \hline
        $MAX\_FLOW\_NUM$ & 65536 \\
        \hline
    \end{tabular}
\end{center}
\fi
\subsubsection{stateful storage}
The details of the usage of stateful storage per flow is listed below. Note that tables like embedding and $GRU$s are excluded since they are not stateful.

\begin{center}
    \begin{tabular}{||c c||}
        \hline
        use & bits/flow $^{*}$ \\ [0.5ex] 
        \hline\hline
        $FlowInfo$ & 64 \\ 
        \hline
        packet counter $^{**}$ & 8+8 \\
        \hline
        last $TS$ $^{***}$ & 32 \\
        \hline
        embedding vector & 8*(S-1) \\
        \hline
        window counter & 8 \\
        \hline
        confidence counter & 16*N \\
        \hline
        escalation mark & 8 \\
        \hline
        \multicolumn{2}{p{.8\linewidth}}{
            \small
            \item Notes. *: Each stateful storage cell should be a multiple of eight bits.
            \item **: The packet counter is implemented by two counters, see Section \ref{subsubsec:counters}.
            \item ***: Limited by hardware, it is necessary to store an additional TS value for the calculation of IPD.
        } \\
    \end{tabular}
\end{center}

With $S=8$ and $N=5$, each flow costs $8S+16N+120$ bits of stateful storage in theory.

\subsubsection{stateless SRAM}
The main SRAM costed by the tables are reported below.

\begin{center}
    \begin{tabular}{||c c||}
        \hline
        SRAM use & cost / total per stage ($\%$) \\ [0.5ex] 
        \hline\hline
        Embed IPD & 5 \\ 
        \hline
        FC & 65 \\ 
        \hline
        first GRU & 1.25 \\
        \hline
        last GRU & 65 \\
        \hline
        middle GRUs & 80\\
        \hline
    \end{tabular}
\end{center}

The key of the first $GRU$ is only consists of $ev_1$, so there are fewer entries. The last $GRU$ is merged with the output layer, so the action data is smaller than other GRUs, i.e., the bit width of intermediate confidence is smaller than the bit width of hidden state.

%\subsubsection{stage usage}
%Limited by the use of stateful storage, the bins to store embedding vectors (see Section \ref{subsubsec:RNN_cell_and_output_layer} and \ref{subsec:impl_of_ev_storage}) cannot be allocated in a single stage, nor can the window counters (see Section \ref{subsubsec:decision_making} and \ref{subsec:impl_of_decision_making}). Also, some tables have to be placed into multiple stages.

%The stage usage is listed below.
\iffalse
\begin{center}
    \begin{tabular}{|| c | c | c ||}
        \hline
        stage & ingress & egress \\ [0.5ex] 
        \hline\hline
        0 & \makecell{$\textsf{calculate}\ ID,\ idx$} & \makecell{$GRU_4$, \\$WindowCounter1$} \\ 
        \hline
        1 & $FlowInfo$ & \makecell{$GRU_5$, \\$\textsf{calculate\ threshold}$} \\ 
        \hline
        2 & \makecell{$pkt\_counter1$, \\$pkt\_counter2$, \\$last\_TS$} & $GRU_5$ \\ 
        \hline
        3 & $\textsf{calculate}\ IPD$ & $GRU_6$ \\ 
        \hline
        4 & $Ebd$ & $GRU_7$ \\ 
        \hline
        5 & $FC$ & $GRU_8$ \\ 
        \hline
        6 & $bin_{3,4,5,6}$ &  \\ 
        \hline
        7 & $bin_{0,1,2}$ & $cnt_0$ \\ 
        \hline
        8 & $\textsf{adjust order}$ & \makecell{$cnt_{1,2,3,4}$, \\ $t\gets argmax(cnt_0,\textsf{threshold})$} \\ 
        \hline
        9 & $GRU_1$ & $argmax(cnt_{1,2,3,4},t)$ \\ 
        \hline
        10 & $GRU_2$ & \\ 
        \hline
        11 & $GRU_3$ & \\ 
        \hline
    \end{tabular}
\end{center}

$GRU_5$ is divided into 2 stages due to the resource sharing between ingress and egress. For the same reason, $cnt_i$s cannot be allocated earlier, such as in stage $6$. The $argmax$ operation is also divided into two parts. The first part is to compare $cnt_0$ and $threshold$, keeping the greater one, denoted as $t$ in the above table. The second part gets the maximum among $cnt_1$ to $cnt_4$ and $t$. The first part costs $4.17\%$ TCAM of the $8^{th}$ stage and the second part costs $58.33\%$ of the $9^{th}$ stage.
\fi

==> ModelDesign/SlidingWindow.tex <==
\subsection{\label{subsec:multi-level} Multi-level Analysis}

Since each RNN time step requires a stage to calculate and the number of stages on the switch is very limited, we use binary RNN as an analysis block for fixed-length flow segment. Specifically, we use a fixed-size window to extract flow segment for binary RNN analysis, and slide this window packet by packet to obtain the analysis results of all possible segments in a flow.

In training, for all possible segments in a flow, binary RNN learns to output an analysis result which is consistent with the flow label. And for traffic analysis on the switch, we integrate the binary RNN analysis results of different segments to make the final decision. In a simple setup, we select the one that contains the most segments among all analysis results for the flow.

Further, to mitigate the accuracy loss caused by switch limitations, we perform multi-level analysis on flow with insufficient result confidence. First, we set a decision threshold to measure the confidence in the flow analysis result. Then, we calculate the proportion of the result containing the most segments and compare it to the decision threshold. If it is smaller than the threshold, we forward the flow to an unconstrained model for further analysis. \notsure{The details of the unconstrained model?}

Moreover, given the sliding window size $S$, the first $S-1$ packets of a flow can not fill the window for binary RNN to analysis. For these packets, we use a Decision Tree (DT) model to perform per-packet analysis after storing their embedding vectors. This DT model is implemented by ternary-matching based on switch TCAMs, and there is no resource competition with the SRAM-based binary RNN model. Finally, we summarize our multi-level analysis workflow in Algorithm~\ref{alg:multi-level}.


==> body_old.tex <==
% \section{Introduction}
% \section{Related Work}
% \section{System Design}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{images/fig model.png}
%     \caption{\label{fig:model} wait to be named.}
% \end{figure}

% \subsection{Model}

% To efficiently handle the sequence of packet information for traffic analysis on switches, we design an RNN-like model.
% Traditional RNN (shown in Figure \ref{fig:model} (a)) cannot be deployed due to the strict restrictions on the usage of stateful memory of switches. RNN requires ‘memory’, which is implemented with registers. One step of the hidden layer of RNN consists of a series of operations: (i) reading prior information from ‘memory’, (ii) calculating new information with prior information and input value, (iii) writing new information back to ‘memory’. The operation (i) and (iii) access the same register, forcing the whole process into a single stage, which is far beyond the capability of switches.

% A natural idea is to unfold the hidden layer of RNN and truncate the length of memory, as shown in Figure \ref{fig:model} (b). This model (denoted as simple unfolded RNN) prevents the duplicate access to a same register, but it is too stage-costly. A model with memory length $N$ requires $2N$ stages, which is obviously unaffordable.

% To save the number of stages, we advanced the model shown as Figure \ref{fig:model} (c). It can be viewed as an unfolded RNN with step $d$. Compared to the simple unfolded RNN, this model saves $d$ times fewer stages at the cost of the increment of calculation complexity of each memory cell ($Mem$ in Figure \ref{fig:model} (c)). Each memory cell can have its own parameters. The calculation function of the value of memory cell $X$ is denoted as $FuncX$.

% \subsection{Algorithm}

% \begin{algorithm}[t]
%   \SetAlgoLined
%   \KwIn{$f$: a single flow, $d$: the step of the model, $N$: the number of steps of the model, $info_{f}$[$i$]: the information of the $i^{th}$ packet of $f$, $mem_{f,X}$[$i$]: the value of memory cell $X$ when calculating the result for the sequence of information from the $(i–N*d+1)^{th}$ packet to the $i^{th}$ packet, $1\le X\le N$, $FuncX$: the calculation function of the value of memory cell $X$, $1\le X\le N$}
%   \KwOut{$result_{i}$: the result for the sequence of information from the $(i–N*d+1)^{th}$ packet to the $i^{th}$ packet}
%   \For{$i$ from 1 to length of $f$}{
%     \If{$i\ge d$}{
%       $mem_{f,1}[i+(N-1)*d]\leftarrow Func1(info_{f}[i-d+1], …, info_{f}[i])$\;
%     }
%     \If{$i\ge 2*d$}{
%       $mem_{f,2}[i+(N-2)*d]\leftarrow Func2(mem_{f,1}[i+(N-2)*d], info_{f}[i-d+1], …, info_{f}[i])$\;
%     }
%     \ldots\;
%     \If{$i\ge N*d$}{
%       $mem_{f,N}[i]\leftarrow FuncN(mem_{f,N-1}[i], info_{f}[i-d+1], …, info_{f}[i])$\;
%       $result_{i}\leftarrow mem_{f,N}[i]$\;
%     }
%   }
%   \caption{The offline algorithm to calculate results for each packet of a flow}
%   \label{algo:offline}
% \end{algorithm}

% Algorithm \ref{algo:offline} describes the processing logic of a single flow. When processing a packet, prior information is used to calculate the current result, say, value of $mem N$, as Line (9) to (12) in Algorithm \ref{algo:offline} describes. Also, some preparatory works should be done for future results (Line (2) to (8) in Algorithm \ref{algo:offline}). After we analyze the lifespan of each value in Algorithm \ref{algo:offline}, we can find that $mem_{f,X}[i]$ is calculated when processing the ${(i-(N-X)*d)}^{th}$ packet (for $1\le X\le N$) and used when processing the ${(i-(N-X+1)*d)}^{th}$ packet (for $1\le X\le N-1$), and $info_{f}[i]$ becomes useless after processing the ${(i+d-1)}^{th}$ packet. As a result, $mem_{f,N}[]$ does not need storage and $mem_{f,X}[i+d]$ can reuse the storage of $mem_{f,X}[i]$ with the operation get-and-modify, so $mem_{f,X}[]$ takes d registers for each $X$ from $1$ to $N-1$ and $mem_{f,N}[]$ does not need stateful storage as it won’t be used by following packets. Similarly, $info_{f}[]$ needs $(d-1)$ registers. These stateful storage costs are linear to the number of supported flows, so the scalability is guaranteed.

% \subsection{\label{sec:flow management} Flow Management}

% The flow index plays an import role in flow management. Prior arts (e.g., FlowLens) rely on control plane to allocate indices for each flow, which is not suitable for line-speed traffic analysis. We compute the flow index based on hash function on data plane. The expression of flow index is $H(5-tuple)\%FLOW\_NUM$, where $H$ is a hash function.

% Hash function will inevitably encounter collisions. To ease this problem, we design a data structure called $Flow Manager$. In $Flow Manager$, each flow stores its flow ID and latest timestamp. When a packet comes, we compute the flow index and flow ID, and check the timestamp in $Flow Manager$ to see whether the stored flow is out of date. If the stored flow is out of date, we replace the timestamp and flow ID with the new packet and refresh the stateful memories in the subsequent processing, whether the flow IDs are equal or not. If the stored flow is still alive, we update the timestamp if the flow IDs are equal, otherwise we fall back to the per-packet analysis for the new packet. Limited by the stateful storage, we cannot store the full 5-tuple as flow ID. Instead, we use another hash function $H^{\prime}$ to compute $H^{\prime}(5-tuple)$ as the flow ID, minimizing the possibility of distraction between different flows.

% The solution above faces difficulty in the flow management across the ingress and the egress. For instance, flow $a$ and flow $b$ do not encounter hash collision in their ingress pipelines $A$ and $B$ respectively, but they are forwarded to the same egress pipeline $C$ and have collision with each other. In this case, the stateful information stored in at least one side of $A$ and $B$ become meaningless, leading to the waste of the precious on-chip memory. Unless there is an one-to-one mapping between ingress pipelines and egress pipelines (i.e., the switch is treated as wires), the flow management will suffer from such cross-pipeline hash collision.

% \section{Implementation}

% \subsection{Hardware Resources}

% To implement the $mem_{f,X}[]$, we allocate an array of $d * FLOW\_NUM$ registers called $memX$ for each $X$ from $1$ to $N-1$, where the $FLOW\_NUM$ is the maximum number of flows we support in the implementation. Then the $mem_{f,X}[i]$ can be transformed into $memX[idx + (i \% d) * FLOW\_NUM]$, where $idx$ is the flow index of $f$, ranging from $0$ to $FLOW\_NUM - 1$.

% There are two approaches to implement $FuncX$. The first one is based on the mechanism of match-action table. Each $FuncX$ is corresponding to a table with input vector as keys and output value as action data, and the only action of the table is writing the output value to metadata. If there are some regularities in the distribution of output value, the table might be compressed with ternary matching. The second one is based on the register with the input vector as index. The space overhead has an exponential relationship with the size of the input vector for both approaches, so the bit width of value of memory cell and packet information cannot be large, neither can the step $d$.

% To implement $info_{f}[]$, we maintain the information of past $d-1$ packets for each flow. There are also two approaches. The first one allocates $d-1$ arrays of $FLOW\_NUM$ registers named $beforeX$ ($1\le X\le d-1$). For a flow $f$ with index $idx$, $beforeX[idx]$ represents the information of the $X^{th}$ packet before the next coming packet of $f$. These arrays are allocated in successive stages and can be updated sequentially when a new packet comes. The second approach also allocates $d-1$ arrays of $FLOW\_NUM$ registers named $binX$ ($1\le X\le d-1$). The information of the $i^{th}$ packet of $f$ is stored in $bin(i\%(d-1))[idx]$. These arrays can be accessed in parallel, at the cost of the dependency on the counter $i\%(d-1)$ and an extra stage to adjust the order of metadata.

% \subsection{Deployment}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{images/fig dependency.png}
%     \caption{\label{fig:depenency} workflow and dependency (the implementation of $info_{f}[]$ is the first approach)}
% \end{figure}

% The whole workflow and data dependency of our model is shown as Figure \ref{fig:depenency}, where the first approach of implementation of info f1[] is displayed. We deploy a prototype with $d=3$, $N=4$, and $FLOW\_NUM=65536$ on a $Tofino$ switch. The information of packets is consisted of packet length and inter-arrival time, which are embedded into $4$ bits separately at first and finally embedded into $4$ bits in total. Also, the bit width of memory cell is $4$. In the first stage, we embed the packet length and calculate the flow index, flow ID and timestamp. In the second stage, we implement the $Flow Manager$. Counters and arrival time of the last packet are in the third stage. The computations of inter-arrival time and index in $memX$ are done in the forth stage. Then the inter-arrival time is embedded in the fifth stage and the final embedding is done in the sixth stage. $before1[]$ and $before2[]$ are in the seventh and eighth stage respectively. $Func1$, $2$, $3$, and $4$ are in the 9th, 11th, 13th, and 15th stage respectively. And $mem1[]$, $mem2[]$, $mem3[]$ are allocated in the 10th, 12th, and 14th stage. On the $Tofino2$ switch, this model can be fully deployed in the ingress pipeline. On the $Tofino$ switch, however, we have to leverage both the ingress and the egress to address the requirement of stages, leading to the limitation discussed in Section \ref{sec:flow management}.

% \section{Evaluation}

% \section{Conclusion}

% \section{Get the maximum value within a single stage}

% The limitation of stages require us to get the maximum value within a single stage. We define the problem as following conditions and restrictions.

% \begin{enumerate}
% \item There are $n$ numbers of $m$ bit(s) each, where $n,m\ge 1$.
% \item There is a predefined order to determine which number to select when there is a tie for maximum value.
% \item Only one ternary matching is allowed, i.e., the calculation before matching is prohibited.
% \end{enumerate}

% We advance an algorithm to design the entries of ternary matching. Firstly, there are two naive cases. For $n=1$, only one entry (i.e., all wildcards) is needed. For $m=1$, we need $n$ entries, i.e., enumerate the winning case of each number in predefined reverse order. For other cases, we first compare the most significant bits and (i) weed out some of the numbers, or (ii) ignore this bit when all bits are equal. Then the problem is reduced to a sub-problem with $m'=m-1$.

% We denote the number of required entries based on our algorithm as $F(n,m)$. The recurrence relations of $F$ is given as follows.

% \begin{equation}
% \label{math:base,m=1}
% F(n,1)=n,n\ge 1
% \end{equation}

% \begin{equation}
% \label{math:base,n=1}
% F(1,m)=1,m\ge 1
% \end{equation}

% \begin{equation}
% \label{math:recursion}
% F(n,m)=F(n,m-1)+\sum_{i=1}^{n-1}\binom{n}{i}F(i,m-1),n\ge 2,m\ge 2
% \end{equation}

% The meaning of \ref{math:recursion} is described as follows. If there are $i$ numbers whose most significant bit is '1', where $1\le i\le n-1$, then we only have to focus on these $i$ numbers, ignoring the rest $n-i$ numbers (i.e., give a wildcard). Otherwise, the most significant bits are all the same, and we ignore this bit (i.e., give a wildcard) and continue with the rest $m-1$ bits for each number.

% The conclusion is that $F(n,m)=nm^{n-1}$. The simplest way to verify it is the mathematical induction. 

% \begin{equation}
% \begin{aligned}
% F(n,m-1)+\sum_{i=1}^{n-1}\binom{n}{i}F(i,m-1)\\
% =\sum_{i=1}^{n}\binom{n}{i}i(m-1)^{i-1}\\
% =n\sum_{i=1}^{n}\binom{n-1}{i-1}(m-1)^{i-1}\\
% =n\sum_{i=0}^{n-1}\binom{n-1}{i}(m-1)^{i}\\
% =nm^{n-1}=F(n,m)
% \end{aligned}
% \end{equation}

% We give another deduction from the equation \ref{math:recursion} as follows. Firstly, let $F(0,m)=0,m\ge 1$, which is consist with the equation \ref{math:base,m=1}. Then the equation \ref{math:recursion} can be write as below.

% \begin{equation}
% F(n,m)=\sum_{i=0}^{n}\binom{n}{i}F(i,m-1),n\ge 0,m\ge 2
% \end{equation}

% We do the deformation to the formula and get:
% \begin{equation}
% F(n,m)=\sum_{i=0}^{n}\frac{n!}{i!(n-i)!}F(i,m-1),n\ge 0,m\ge 2
% \end{equation}

% \begin{equation}
% \label{math:deformation}
% \frac{F(n,m)}{n!}=\sum_{i=0}^{n}\frac{F(i,m-1)}{i!}\frac{1}{(n-i)!},n\ge 0,m\ge 2
% \end{equation}

% We denote $\frac{F(n,m)}{n!}$ as $^{m}g_n$, and $\frac{1}{n!}$ as $h_n$. Then we construct the generating function of $^{m}g$ and $h$.

% \begin{equation}
% \label{math:generation,g}
% ^{m}G(x)=\sum_{n=0} {^{m}g_{n}}x^n=\sum_{n=0}\frac{F(n,m)}{n!}x^n,m\ge 1
% \end{equation}

% \begin{equation}
% H(x)=\sum_{n=0}h_{n}x^n=\sum_{n=0}\frac{x^n}{n!}=e^x
% \end{equation}

% We can obtain the recursive relations between $^{m}G$ and $^{m-1}G$ from equation \ref{math:deformation}.

% \begin{equation}
% ^{m}G=^{m-1}G\times H,m\ge 2
% \end{equation}

% And for $m=1$, we have

% \begin{equation}
% \begin{aligned}
% ^{1}G(x)=\sum_{n=0} {^{1}g_{n}}x^n=\sum_{n=0}\frac{F(n,1)}{n!}x^n\\
% =\sum_{n=0}\frac{n}{n!}x^n=\sum_{n=1}\frac{1}{(n-1)!}x^n\\
% =x\sum_{n=0}\frac{1}{n!}x^n=xe^x
% \end{aligned}
% \end{equation}

% With the mathematical induction, we can get

% \begin{equation}
% ^{m}G(x)=xe^{mx},m\ge 1
% \end{equation}

% Compared with the equation \ref{math:generation,g} and we can get

% \begin{equation}
% \begin{aligned}
% F(n,m)=^{m}G^{(n)}(0)=(x e^{m x})^{(n)}\bigg|_{x=0}\\
% =(n m^{n-1}+m^n x)e^{m x}\bigg|_{x=0}\\
% =nm^{n-1},n\ge 1,m\ge 1
% \end{aligned}
% \end{equation}

% QED.

% If there are two or more stages available, we can do subtraction between every two numbers at the first stage and then do ternary matching based on the sign bits with only $n$ entries.

==> discussion.tex <==
\section{Discussion}

\fixme{Hardware Agnostic.} 
The key designs of \sys are sliding-window based RNN realization and table-based on model deployment on hardware. 
Table-matching is the universal primitive for any programmable dataplane. 
Thus, we expect our designs, with lightweight adaptation, are also deployable on programmable switches other than Tofino. 
